Efficiently Forgetting What You Have Learned in Graph Representation Learning via Projection

As privacy protection receives much attention, unlearning the effect of a specific node from a pre-trained graph learning model has become equally important. However, due to the node dependency in the graph-structured data, representation unlearning in Graph Neural Networks (GNNs) is challenging and less well explored. In this paper, we fill in this gap by first studying the unlearning problem in linear-GNNs, and then introducing its extension to non-linear structures. Given a set of nodes to unlearn, we propose PROJECTOR that unlearns by projecting the weight parameters of the pre-trained model onto a subspace that is irrelevant to features of the nodes to be forgotten. PROJECTOR could overcome the challenges caused by node dependency and enjoys a perfect data removal, i.e., the unlearned model parameters do not contain any information about the unlearned node features which is guaranteed by algorithmic construction. Empirical results on real-world datasets illustrate the effectiveness and efficiency of PROJECTOR.

==> sections/expressive_power.tex <==


\subsection{An alternative view on the limitation of graph convolution in linear GNN}

Study graph representation learning through the lens of linear GNN via logistic regression gives us an alternative view and novel understanding on the over-smoothing effect in GNN training.
For the ease of presentation, we only consider the $c$-th channel of the trained weight matrix $\mathbf{W}$, which is denoted as 
\begin{equation}
    \mathbf{w}_c = \sum_{i=1}^N \gamma_i y_{i,c} \mathbf{h}_i = \sum_{i=1}^N \gamma_i y_{i,c} \Big(\sum_{j=1}^N p_{ij}\mathbf{x}_j \Big), 
\end{equation}
for a set of coordinate constants $\{\gamma_i\}_{i=1}^N$.
During evaluation, the prediction on the $i$-th data point is predicted as $p_{c,k}  = \text{sigmoid}(\mathbf{w}_c^\top \mathbf{h}_k )$ which can be regarded as comparing the similarity between node representation $\mathbf{h}_k$ with all the training node representation $\{ \mathbf{h}_1, \ldots, \mathbf{h}_N\}$. To see this, we can rewrite $\mathbf{w}_c \mathbf{h}_k$ as 
\begin{equation}
    \mathbf{w}_c^\top \mathbf{h}_k= \Big( \sum_{i=1}^N \gamma_i y_{i,c} \mathbf{h}_i \Big)^\top \mathbf{h}_k=  \sum_{i=1}^N \gamma_i y_{i,c}  \langle \mathbf{h}_i, \mathbf{h}_k \rangle
\end{equation}
The prediction on $\mathbf{h}_i$ is based on the similarity of $\mathbf{h}_i$ to all other node representations $\{ \mathbf{h}_1,\ldots, \mathbf{h}_N \}$, which is measured by the inner product of two node representations.

\begin{proposition} \label{proposition:our_goal_on_P}
To achieve prediction with high accuracy, we are expecting $\langle \mathbf{h}_i, \mathbf{h}_k \rangle$ is as large as possible if they belongs to the same category; $\langle \mathbf{h}_i, \mathbf{h}_k \rangle$ is as less as possible if they belongs to the different category.
\end{proposition}

Recall that node representation $\mathbf{h}_i = \sum_{j=1}^N p_{ij} \mathbf{x}_j$, as a result, we know that $ \langle \mathbf{h}_i, \mathbf{h}_k \rangle$ can be think of as comparing the neighborhood node features of node $i$ and node $k$ by computing the inner-product of each node pairs.
\begin{equation}
    \langle \mathbf{h}_i, \mathbf{h}_k \rangle = \Big\langle \sum_{j=1}^N p_{ij} \mathbf{x}_j, \sum_{l=1}^N p_{kl} \mathbf{x}_l \Big\rangle = \sum_{j=1}^N \sum_{l=1}^N p_{ij}p_{kl} \langle \mathbf{x}_j, \mathbf{x}_l \rangle 
\end{equation}



Therefore, to achieve our goal in Proposition~\ref{proposition:our_goal_on_P}, we have to design the graph propagation matrix $\mathbf{P}(\mathbf{A})$ by taking both the node label and node features into consideration: \textcolor{red}{this part is not accurate ...}
\begin{itemize} [noitemsep,topsep=0pt,leftmargin=3mm ]
    \item If node $v_i, v_k$ belong to the \emph{same} category (i.e., $y_{i,c} = y_{k,c}$), then for any two node $v_j, v_l$  feature
    \begin{itemize}[noitemsep,topsep=0pt,leftmargin=3mm ]
        \item if $\langle \mathbf{x}_j,~\mathbf{x}_l\rangle$ is large, then we expect $p_{ij},p_{kl}$ to be large;
        \item if $\langle \mathbf{x}_j,~\mathbf{x}_l\rangle$ is small, then we expect $p_{ij},p_{kl}$ to be small;
    \end{itemize}
    \item If node $v_i, v_k$ belong to the \emph{different} category (i.e., $y_{i,c} \neq y_{k,c}$), then for any two node $v_j, v_l$  feature
    \begin{itemize}[noitemsep,topsep=0pt,leftmargin=3mm ]
        \item if $\langle \mathbf{x}_j,~\mathbf{x}_l\rangle$ is large, then we expect $p_{ij},p_{kl}$ to be small;
        \item if $\langle \mathbf{x}_j,~\mathbf{x}_l\rangle$ is small, then we expect $p_{ij},p_{kl}$ to be large;
    \end{itemize}
\end{itemize}
which is different from the existing graph in linear GNN that only take the graph structure into consideration.


In fact, the idea of considering both node features and label information for graph propagation has been widely used in
self-attention based GNNs (non-linear GNN with activation functions and weight matrices at each layer) for many years. In self-attention based GNNs, the self-attention value is computed on the node features using weight inner product, therefore they also take the node feature into consideration. Meanwhile, during training, the label information can be propagated to the GNN model by updating the weight matrices in the self-attention module, which can be regarded as also taking the label information into consideration.

Although empirical results suggests that self-attention based GNNs are powerful, employing self-attention mechanism in linear GNN (here we need linear GNN because of its advantage in unlearning and scalable training) is non-trivial.
In the next section, we introduce a method to train such propagation matrix for linear GNN under the notation of diffusion equation, which has been widely used in image processing and recently gain many attention in graph representation learning.


\textcolor{red}{the above also provide an alternative explainable on over-smoothing effect in linear GNN but not ordinary gnn }

\subsection{Context-guided diffusion on graph}


We propose our solution under the notation of continuous-depth GNN motivated by its memory-efficient property and its ability to model the dynamics of hidden layers more smoothly. 

\noindent\textbf{Diffusion equation on graph.}~
Before diving into details, let first introduce notations that will be used in the following discussion.
Let $\mathbf{X}(t) = [\mathbf{x}_1(t), \ldots, \mathbf{x}_N(t)] \in \mathbb{R}^{N\times d}$ denote the features of each node at the continuous-depth $t$.
% Let $\mathbf{A}\in\mathbb{R}^{N\times N}$ be a symmetric matrix where $A_{ij}=A_{ji} \in \mathbb{R}$ represents the edge weight between node $i$ and node $j$ and $A_{ij}=0$ if edge does not exist.
Let $\nabla \mathbf{X}(t) \in \mathbb{R}^{N\times N\times d}$ as the gradient operator on $\mathbf{X}(t)$, where $[\nabla \mathbf{X}(t)]_{i,j,\star} = \mathbf{x}_j(t) - \mathbf{x}_i(t)$.
Let $\mathbf{D}(\mathcal{G}(t), t) \in \mathbb{R}^{N\times N}$ be an algorithm dependent diffusion operator, where the diffusion operation is applied to $\nabla \mathbf{X}$ and the computation of each element $D_{ij}(\mathcal{G}(t), t) \in \mathbb{R}$ will be elaborate later. 
Let $\mathcal{X}(t) = \mathbf{D}(\mathcal{G}(t), t) \odot \nabla \mathbf{X}\in \mathbb{R}^{N\times N\times d}$ denote the feature of each edge at the continuous-depth $t$. The divergence operator is applied on edge features $\text{div}(\mathcal{X}(t)) \in \mathbb{R}^{N\times d}$ with $[\text{div}(\mathcal{X}(t))]_i = \sum_{j=1}^N A_{ij} [\mathcal{X}(t)]_{i,j,\star}$ and $A_{ij}$ is the $i$-th row and $j$-th column of adjacency matrix $\mathbf{A}$.
Then, the following diffusion process that evolves the feature matrix $\mathbf{X}$ on the graph is computed as
\begin{equation}
    \frac{\partial \mathbf{X}(t)}{\partial t} = \text{div}\left( \mathbf{D}(\mathcal{G}(t), t) \odot \nabla \mathbf{X}(t) \right) =  (\mathbf{D}(\mathcal{G}(t),t) - \mathbf{I}) \mathbf{X}(t)
\end{equation}
The node representation at continuous-depth $T$ can be computed by
\begin{equation}
    \mathbf{X}(T) = \mathbf{X}(0) + \int_{0}^T \frac{\partial \mathbf{X}(t)}{\partial t} dt,~\text{with}~\mathbf{X}(0) = \mathbf{X}.
\end{equation}

\noindent\textbf{Diffusion operator in different algorithms.}~
In the simplest case when $\mathbf{D}(\mathcal{G}(t), t)$ is only dependent on the graph structure, e.g., $\mathbf{D}(\mathcal{G}(t), t) = \mathbf{P}_\text{row}$ or $\mathbf{P}(\mathcal{G}(t), t) = \mathbf{P}_\text{sym}$, the solution is reduced to a continuous-step GCN.
Besides, \textit{GRAND}~\cite{chamberlain2021grand} adopt a feature and time-step dependent diffusion operator, where $\mathbf{D}(\mathcal{G}(t), t)$ is the multi-head self-attention~\cite{velivckovic2017graph} computed on $\mathbf{X}(t)$.~\textit{BLEND}~\cite{chamberlain2021beltrami} utilize the same diffusion operator as~\cite{chamberlain2021grand} but a different feature initialization, i.e., $\mathbf{X}(0) = [\mathbf{X}, \mathbf{U}]$ where $\mathbf{U}$ is a trainable positional encoding of each node.
\textit{GRAND++}~\cite{thorpe2021grand++} adds a source term on top of~\cite{chamberlain2021grand} to alleviate the over-smoothing effect.
Although~\cite{chamberlain2021grand,thorpe2021grand++,chamberlain2021beltrami} are powerful, these methods are not ideal for graph representation unlearning because unlearn the information related to the deleted node features from the weight matrices in the multi-head self-attention module is non-trivial.


\noindent\textbf{Context-guided diffusion on graph.}~
We propose to take both the node feature and label information into consideration:
\begin{equation}
    [\mathbf{X}, \mathbf{Y}](T) = [\mathbf{X}, \mathbf{Y}](0) + \int_{0}^T \frac{\partial [\mathbf{X}, \mathbf{Y}](t)}{\partial t} dt,~\text{with}~[\mathbf{X}(0), \mathbf{Y}(0)] = [\mathbf{X}, (\mathbf{P}-\text{diag}(\mathbf{P}))\mathbf{Y}].
\end{equation}
where $\text{diag}(\mathbf{P})$ is the diagonal matrix of $\mathbf{P}$ and $\mathbf{P}$ can be either $\mathbf{P}_\text{row}$ or $\mathbf{P}_\text{row}$ depending on the dataset. 
The diffusion operator is computed by taking the similarity of node feature and label category into consideration.
For example, one can define the propagation matrix as 
\begin{equation}
    D_{ij}(\mathcal{G}(t), t) = \frac{\omega_{ij}}{\sum_{k=1}^N \omega_{ik} },~\text{where}~
    \omega_{ij} = \exp\left( - \frac{\| \mathbf{x}_i(t) - \mathbf{x}_j(t) \|_2^2}{\sigma_x^2} - \frac{\| \mathbf{y}_i(t) - \mathbf{y}_j(t) \|_2^2}{\sigma_y^2} \right),
\end{equation}
and $\sigma_x, \sigma_y \in \mathbb{R}$ are parameters learned during training.


and the above formula has connection to do with the Graph Attention Networks.




==> sections/graph_conv_non_linear.tex <==
% In this section, we introduce an unlearning favorable adaptive diffusion for graph in Section~\ref{section:context_guide_diffusion} and an unlearning favorable extension from linear GNN to non-linear GNN in Section~\ref{section:extension_non_linear}.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \subsection{Adaptive diffusion on graph} \label{section:context_guide_diffusion}

% \textcolor{red}{motivation: In image processing, one can exploit this interpretation of diffusion as linear low-pass filtering for image denoising. However, such a filter, when removing noise, also undesirably blurs transitions between regions of different color or brightness (``edges''). An influential insight of Pietro Perona and Jitendra Malik [5] was to consider an adaptive diffusivity coefficient inversely dependent on the norm of the image gradient $|\nabla x|$. This way, diffusion is strong in “flat” regions (where $|\nabla x|\approx 0$) and weak in the presence of brightness discontinuities (where $|\nabla x|$ is large). The result was a nonlinear filter capable of removing noise from the image while preserving edges.}
% \textcolor{red}{we can remove the integral thing and only consider that Euler approximation is fine}

% \textcolor{blue}{For instance, in image processing, diffusivity is strong in flat regions but weaker on edges. Further, on an edge, diffusivity is stronger along the direction of edges than across it. This leads to edge-preserving image smoothing as pioneered by Weicker}

% We propose our solution under the notation of continuous-depth GNN motivated by its memory-efficient property and its ability to model the dynamics of hidden layers more smoothly. 

% \noindent\textbf{Diffusion in graph.}~
% In image processing, diffusion has been interpreted as linear low-pass filtering for image demonising. However, diffusion can undesirably blurs neighborhood regions of different color and brightness. \cite{perona1990scale} propose an edge-preserving diffusion method by taking the difference of the pixels to be diffused into consideration, i.e., diffusion is strong if the difference is small (e.g., flat region or along edge) but weaker if the difference is large (e.g., across edges). 
% Recently, the edge-preserving diffusion idea has been extended to graph domain aiming at alleviating the over-smoothing issue and build more powerful aggregation schema~\cite{chamberlain2021grand,chamberlain2021beltrami,thorpe2021grand++}.
% %
% For instance, explicit Euler approximation graph diffusion is defined as $\mathbf{H}^{(\ell+1)} = \big( (1-\gamma) \mathbf{I} + \gamma \mathbf{D}^{(\ell)}_\mathcal{G} \big) \mathbf{H}^{(\ell)},$
% \begin{equation}
%     \frac{\mathbf{H}^{(\ell+1)} - \mathbf{H}^{(\ell)} }{\gamma} = (\mathbf{D}^{(\ell)}_\mathcal{G} - \mathbf{I} ) \mathbf{H}^{(\ell)} \Rightarrow \mathbf{H}^{(\ell+1)} = \big( (1-\gamma) \mathbf{I} + \gamma \mathbf{D}^{(\ell)}_\mathcal{G} \big) \mathbf{H}^{(\ell)},
% \end{equation}
% where $\smash{\mathbf{H}^{(\ell)} \in \mathbb{R}^{n\times d}}$ denotes the node features after $\ell$-steps of diffusion, $\gamma$ is the discretization interval, and 
% $\smash{\mathbf{D}^{(\ell)}_\mathcal{G} \in \mathbb{R}^{n\times n}}$ is  an algorithm dependent diffusion operator. 
% When $\gamma=1$, it recovers the linear GNN structure.
% \noindent\textbf{Diffusion equation on graph.}~
% Before diving into details, let first introduce notations that will be used in the following discussion.
% Let $\mathbf{X} = [\mathbf{x}_1, \ldots, \mathbf{x}_N] \in \mathbb{R}^{N\times d}$ denote the features of each node at the continuous-depth $t$.
% Let $\mathbf{A}\in\mathbb{R}^{N\times N}$ be a symmetric matrix where $A_{ij}=A_{ji} \in \mathbb{R}$ represents the edge weight between node $i$ and node $j$ and $A_{ij}=0$ if edge does not exist.
% Let $\nabla \mathbf{X} \in \mathbb{R}^{N\times N\times d}$ as the gradient operator on node features $\mathbf{X}$, where $[\nabla \mathbf{X}]_{i,j,\star} = \mathbf{x}_j - \mathbf{x}_i$.
% Let $\mathbf{D}^{(\ell)}_\mathcal{G} \in \mathbb{R}^{N\times N}$ be an algorithm dependent diffusion operator, where the diffusion operation is applied to $\nabla \mathbf{X}$ and the computation of each element $D_{ij}(\mathcal{G}) \in \mathbb{R}$ will be elaborate later. 
% Let $\mathcal{X} = \mathbf{D}^{(\ell)}_\mathcal{G} \odot \nabla \mathbf{X}\in \mathbb{R}^{N\times N\times d}$ denote the feature of each edge. The divergence operator is applied on edge features $\text{div}(\mathcal{X}) \in \mathbb{R}^{N\times d}$ with $[\text{div}(\mathcal{X})]_i = \sum_{j=1}^N A_{ij} [\mathcal{X}]_{i,j,\star}$ and $A_{ij}$ is the $i$-th row and $j$-th column of adjacency matrix $\mathbf{A}$.
% Then, the following diffusion process that evolves the feature matrix $\mathbf{X}$ on the graph is computed as
% \begin{equation}
%     \frac{\partial \mathbf{X}}{\partial t} = \text{div}\left( \mathbf{D}^{(\ell)}_\mathcal{G} \odot \nabla \mathbf{X} \right) =  (\mathbf{D}^{(\ell)}_\mathcal{G} - \mathbf{I}) \mathbf{X}
% \end{equation}
% The node representation at continuous-depth $T$ can be computed by
% \begin{equation}
%     \mathbf{X} = \mathbf{X}(0) + \int_{0}^T \frac{\partial \mathbf{X}}{\partial t} dt,~\text{with}~\mathbf{X}(0) = \mathbf{X}.
% \end{equation}
%
% \noindent\textbf{Diffusion operator in different algorithms.}~
% For example when $\gamma=1$ and $\smash{\mathbf{D}^{(\ell)}_\mathcal{G} = \mathbf{D}^{-1}\mathbf{A}}$, 
% is only dependent on the graph structure, 
% e.g., $\mathbf{P}(\mathcal{G}) = \mathbf{P}$,
% the solution is reduced to a linear GNN.
% \textsc{Grand}~\cite{chamberlain2021grand,thorpe2021grand++} initialize feature as $\mathbf{H}^{(0)} = \mathbf{X}$ and set diffusion operator  $\smash{\mathbf{D}^{(\ell)}_\mathcal{G}}$ as the multi-head self-attention~\cite{velivckovic2017graph} computed on $\mathbf{H}^{(\ell)}$.~\textsc{Blend}~\cite{chamberlain2021beltrami} utilize the same diffusion operator as \textsc{Grand} but a different feature initialization, i.e., $\mathbf{H}^{(0)} = [\mathbf{X}, \mathbf{U}]$ with $\mathbf{U}$ as a trainable positional encoding of each node.
% \textsc{Grand++}~\cite{thorpe2021grand++} adds a source term on top of \textsc{Grand} to alleviate the over-smoothing effect.
% Although~\cite{chamberlain2021grand,thorpe2021grand++,chamberlain2021beltrami} are powerful, these methods are not ideal for graph unlearning because perfectly remove the sensitive information from the weight parameters of multi-head self-attention module is non-trivial.

Linear GNNs have fixed graph convolution operation that might not fully take advantages of the graph structure.
% \noindent\textbf{An unlearning favorable adaptive diffusion operator.}~
To alleviate this issue, 
% \noindent\textbf{Context-guided diffusion on graph.}~
we propose an unlearning favorable adaptive diffusion operation that take
% both the node feature and label information into consideration.
% \begin{equation}
%     [\mathbf{X}, \mathbf{Y}] = [\mathbf{X}, \mathbf{Y}](0) + \int_{0}^T \frac{\partial [\mathbf{X}, \mathbf{Y}]}{\partial t} dt,~\text{with}~[\mathbf{X}(0), \mathbf{Y}(0)] = [\mathbf{X},\mathbf{Y}].
% \end{equation}
% where $\text{diag}(\mathbf{P})$ is the diagonal matrix of $\mathbf{P}$ and $\mathbf{P}$ can be either $\mathbf{P}_\text{row}$ or $\mathbf{P}_\text{row}$ depending on the dataset. 
% The diffusion operator is computed by taking 
the similarity of both node feature and node label category information into consideration. Let us initialize features as $\smash{\mathbf{h}_i^{(0)} = \mathbf{x}_i}$, initialize labels as $\smash{\mathbf{z}_i^{(0)} = \mathbf{y}_i}$ if $\smash{i\not\in\mathcal{V}_\text{test}}$, and initialize $\smash{\mathbf{z}_i^{(0)} = \mathbf{0}}$ if $\smash{i\in\mathcal{V}_\text{test}}$. Then, the forward propagate is computed as $\smash{[\mathbf{H}^{(\ell+1)}, \mathbf{Z}^{(\ell+1)}] = \big( (1-\gamma) \mathbf{I} + \gamma \mathbf{D}^{(\ell)}_\mathcal{G} \big) [\mathbf{H}^{(\ell)}, \mathbf{Z}^{(\ell)}]}$, where $[\cdot,\cdot]$ is feature dimension concatenation operation and the $i$-th row $j$-th column of the $\ell$-th diffusion operator is defined by 
\vspace{-1.5mm}
\begin{equation} \label{eq:adaptive_diffusion}
    \left[ \mathbf{D}^{(\ell)}(\mathcal{G}) \right]_{i,j} = \frac{\omega_{ij}}{\sum_{k=1}^N \omega_{ik} },~
    \omega_{ij} = \exp\Big( - \frac{\| \mathbf{h}_i^{(\ell)} - \mathbf{h}_j^{(\ell)} \|_2^2}{\sigma_h^2} - \frac{\| \mathbf{z}_i^{(\ell)} - \mathbf{z}_j^{(\ell)} \|_2^2}{\sigma_z^2} \Big),
\end{equation}
and $\sigma_h, \sigma_z \in \mathbb{R}$ are parameters learned during training. Intuitively, our diffusion operator assign a higher neighbor aggregation weight to a node if it has a similar node feature and label information.
Then, we set $\mathbf{H} = [\mathbf{H}^{(L)}, \mathbf{Z}^{(L)}]$ as the final node representation for prediction.
During unlearning, we do not have to modify $\sigma_h, \sigma_z$ since these scalars will not leak the node feature information.
% and the above formula has connection to do with the Graph Attention Networks.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/method_backup.tex <==

In this section, we introduce \our by first preliminaries on graph representation unlearning in Section~\ref{section:preliminary}, then demonstrating its application to graph representation unlearning in Section~\ref{section:application_to_graph} and summarize \our in Algorithm~\ref{alg:projector}, introducing an unlearning-favorable adaptive graph convolution in Section~\ref{section:extension}, and theoretically analyzing its  effectiveness in Section~\ref{section:effectiveness_of_ours}.


\subsection{Preliminary on Graph Representation Unlearning} \label{section:preliminary}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We consider solving the semi-supervised binary node classification problem using the linear GNN structure as proposed in~\cite{wu2019simplifying}, which could be easily extended to multi-class classification by using either cross-entropy loss or under one-over-rest setting.
More specifically, given a graph $\mathcal{G}(\mathcal{V},\mathcal{E})$ with $n=|\mathcal{V}|$ nodes and $|\mathcal{E}|$ edges, let us suppose each node $v_i \in \mathcal{V}$ is associated with node feature vector $\mathbf{x}_i \in \mathbb{R}^{d}$. 
Let $\mathbf{A}, \mathbf{D} \in \mathbb{R}^{n\times n}$ denote the adjacency matrix and its associated degree matrix, respectively. Then, a $L$-layer linear GNN computes the node representation $\mathbf{H} = \mathbf{P}^L \mathbf{X}$ by applying $L$ propagation matrices $\mathbf{P} = \mathbf{D}^{-1}\mathbf{A}$ to the node features matrix $\mathbf{X} \in \mathbb{R}^{n \times d}$.
During training, only training set nodes $\mathcal{V}_\text{train}\subset \mathcal{V}$ are labeled by a binary label $y_i\in\{-1,+1\}$ and our goal is to estimate the label of the unlabeled nodes $\mathcal{V}_\text{eval}=\mathcal{V}\setminus \mathcal{V}_\text{train}$.
More specifically, we want to find the weight parameters $\mathbf{w} \in\mathbb{R}^d$ that minimize 
\begin{equation} \label{eq:ovr_logistic_regression}
    F(\mathbf{w}) = \frac{\lambda}{2} \| \mathbf{w} \|_\mathrm{2}^2 + \frac{1}{\mathcal{V}_\text{train}}\sum_{v_i\in\mathcal{V}_\text{train}} f_i(\mathbf{w}),~
    f_i(\mathbf{w}) = \log\left(1 + \exp(- y_i \mathbf{w}^\top \mathbf{h}_i) \right),\mathbf{h}_i = [\mathbf{P}^L \mathbf{X}]_i
\end{equation}
For graph representation unlearning, let $\mathcal{V}_\text{delete}\subset \mathcal{V}_\text{train}$ denote the set of deleted nodes and $\mathcal{V}_\text{remain} = \mathcal{V}_\text{train} \setminus \mathcal{V}_\text{delete}$ denote the remaining nodes. Our goal is to unlearn the node feature information $\{ \mathbf{x}_i~|~v_i \in \mathcal{V}_\text{delete}\}$ of the deleted nodes $\mathcal{V}_\text{delete}$ from the weight parameters.

\subsection{Application to Graph Data and Bypass Node Dependency} \label{section:application_to_graph}



In the following, we show in Proposition~\ref{prop:logistic_regression_linear_span} that \our can bypass the node dependency issue because the graph convolution in the linear GNN is a linear operator on node features.
% because the graph convolutions in linear GNN can be considered as a weighted combination of node features, such that the weight parameters of linear GNN is a linear combination of node features.
\begin{proposition} \label{prop:logistic_regression_linear_span}
Let us suppose optimizing linear GNN (in Eq.~\ref{eq:ovr_logistic_regression}) using mini-batch SGD with weight initialization satisfying  $\mathbf{w}_\text{init}\in\text{span}\{\mathbf{x}_1,\ldots,\mathbf{x}_n\} $. Then, after $T$-steps of gradient updates we still have $\mathbf{w}(T)\in\text{span}\{\mathbf{x}_1,\ldots,\mathbf{x}_n\}$ holds.
\end{proposition}
To see this, let us first recall the gradient of Eq.~\ref{eq:ovr_logistic_regression} with respect to any $\mathbf{w}$, which is computed as
\begin{equation}\label{eq:grad_linear_gnn_logistic_regression}
    \nabla F(\mathbf{w}) = \lambda \mathbf{w} + \frac{1}{|\mathcal{V}_\text{train}|}\sum\nolimits_{j\in\mathcal{V}_\text{train}} \alpha_j \mathbf{x}_j,~\alpha_j =  \sum\nolimits_{i\in\mathcal{V}_\text{train}} \mu_i [\mathbf{P}^L]_{ij},~
    \mu_i = - y_i \sigma(-y_i \mathbf{w}^\top \mathbf{h}_i),
\end{equation}
where $[\mathbf{P}^L]_{ij}$ denote the $i$-th row $j$-th column of $\mathbf{P}^L$ and $\sigma(\cdot)$ is the sigmoid function.
The Eq.~\ref{eq:grad_linear_gnn_logistic_regression} implies that the gradient lies in the linear span of node features, i.e., $\nabla F(\mathbf{w}) \in \text{span}\{\mathbf{x}_1,\ldots,\mathbf{x}_n\}$. Therefore, when using update rule $\mathbf{w}(t+1) = \mathbf{w}(t) - \eta \nabla F(\mathbf{w}(t))$, the weight % after any $T$ update steps 
after gradient updates still stays inside the subspace defined by the linear span of node features.
% In practice, we use SGD with momentum for training, which has the above observation hold.
From Eq.~\ref{eq:grad_linear_gnn_logistic_regression}, we know that node dependency is included inside the finite sum weight $\alpha_j$, which is a constant that is multiplied with its features $\mathbf{x}_j$. Therefore, we can bypass the node dependency and remove the sensitive information of the deleted node features by projecting the weight onto a subspace that is spanned by the remaining node features $\mathbf{X}_\text{remain}$, where the subspace is irrelevant to the deleted node features $\mathbf{X}_\text{delete}$ as described in the previous section.

To this end, we summarize \our in Algorithm~\ref{alg:projector}. In particular, two different types of input options are available that leads to the identity results: we can use option 1 when only remaining node features are available, otherwise we can use option 2 to computer the projection matrix if only deleted node features are available and pre-computing is feasible.

% One of the key advantages of \our is that it can bypass the node dependency issue and enjoys a relatively lower computation cost that is independent to the number of the GNN layers.
% \textcolor{red}{Appendix~\ref{section:why_bypass} provides further insight on why dependency are bypassed.}
% \our can be easily extended to multi-class classification by using cross-entropy loss. 
% In Section~\ref{section:extension}, we will introduce its extension to a non-linear structure and a more powerful graph convolution operation.

% \begin{wrapfigure}{r}{0.5\textwidth}
% \end{wrapfigure}


\input{supplementary/baseline_methods}


\subsection{On the effectiveness of \our}\label{section:effectiveness_of_ours}
In this section, we study the effectiveness of \our by measuring the $\ell_2$-norm on the difference between $\mathbf{w}_p$ (\oure's output) to $\mathbf{w}_u$ (the solution obtained by retraining from scratch) on the dataset without the deleted nodes. Intuitively, we are expecting $\|\mathbf{w}_p -  \mathbf{w}_u \|_2$ to be small.
% We note that the closeness of weight parameters not necessarily guarantees certified data removal as shown in Theorem~\ref{thm:unlearn_without_change}. 
% For simplicity, we consider training linear GNN in Eq.~\ref{eq:ovr_logistic_regression} with $\lambda=0$.
For unlearning, we suppose a random subset of nodes $\mathcal{V}_\text{delete} \subset \mathcal{V}_\text{train}$ are selected and the remaining nodes are denoted as $\mathcal{V}_\text{remain} = \mathcal{V}_\text{train}  \setminus \mathcal{V}_\text{delete} $. 
% For notation simplicity, let suppose we reorder the nodes such that all the deleted nodes $\mathcal{V}_\text{delete}$ are placed in the front of all nodes.
Notice that removing the nodes $\mathcal{V}_\text{delete}$ is the same as updating the propagation matrix from $\mathbf{P}$ to $\mathbf{P}_u$, where all edges that are connected to node $v_i\in\mathcal{V}_\text{delete}$ are removed in $\mathbf{P}_u$. Therefore, we can write down the objective after data deletion $F^u(\mathbf{w}_u) $ as
% \begin{equation} \label{eq:closeness_after_delete_objective}
%     \begin{aligned}
%     \min_{\mathbf{w}_u \in \mathbb{R}^d}~F^u(\mathbf{w}_u) 
%     &= \frac{1}{|\mathcal{V}_\text{remain}|}\sum_{i\in\mathcal{V}_\text{remain}} f_i^u(\mathbf{w}_u) \\
%     \text{where}~f_i^u(\mathbf{w}_u) &= \log\left( 1 + \exp(-y_i \mathbf{w}_u^\top \mathbf{h}^u_i) \right), \mathbf{h}^u_i = [\mathbf{P}_u^L \mathbf{X}]_i.
%     \end{aligned}
% \end{equation}
\begin{equation} \label{eq:closeness_after_delete_objective}
    \min_{\mathbf{w}_u \in \mathbb{R}^d}F^u(\mathbf{w}_u) = \frac{1}{|\mathcal{V}_\text{remain}|}\sum_{v_i\in\mathcal{V}_\text{remain}} f_i^u(\mathbf{w}_u),
    f_i^u(\mathbf{w}_u) = \log\left( 1 + \exp(-y_i \mathbf{w}_u^\top \mathbf{h}^u_i) \right) + \lambda \| \mathbf{w}_u\|_2,~
\end{equation}
where $\mathbf{h}^u_i = [\mathbf{P}_u^L \mathbf{X}]_i$.
Let $\mathbf{w}(t),~\mathbf{w}_u(t)$ denote the weight parameters obtained by using full-batch GD training from scratch on $\mathcal{V}_\text{train},~\mathcal{V}_\text{remain}$ for $t$ epochs with the same initialization $\mathbf{w}(0) = \mathbf{w}_u(0)$, and $\mathbf{w}_p(t)$ denote the weight parameters obtained by applying \our on $\mathbf{w}(t)$.

% We make the following assumptions on the propagation matrices, weight parameters, and node features.

Before proceeding to our result, we make the following customery assumptions on graph propagation matrices, node features, and weight matrices  in Assumption~\ref{assumption:upper_bound_on_node_feats}, on the variance of stochastic gradients in Assumption~\ref{assumption:expectation_random_delete_nodes}, and on the correlation between node feature in Assumption~\ref{assumption:upper_bound_on_approximation_error}. Please notice that Assumption~\ref{assumption:upper_bound_on_node_feats},~\ref{assumption:expectation_random_delete_nodes} are standard assumptions in GNN's theoretical analysis~\cite{cong2021provable,ramezani2021learn} and Assumption~\ref{assumption:upper_bound_on_approximation_error} is mild assumptions that could be empirically verified in Table~\ref{table:delta_on_real_world}.

\weilin{$\delta$ can be think of as a measurement on the closeness of the subspace defined with and without the deleted node features.}

\begin{assumption}\label{assumption:upper_bound_on_node_feats}
We assume each row of each propagation matrices before and after node deletion are bounded by $P_s\geq0$, i.e., $\max_j \left\| [ \mathbf{P}^L ]_j \right\|_2 \leq P_s, ~\max_j \left\| [ \mathbf{P}^L_u ]_j \right\|_2 \leq P_s$.
Besides, we assume the row of the difference of the propagation matrices before and after data deletion is bounded by $P_d\geq0$, i.e., $\max_j \left\| [ \mathbf{P}^L_u - \mathbf{P}^L ]_j \right\|_2 \leq P_d$.
Furthermore, we assume the norm of any node features $\mathbf{x}_i,~v_i\in\mathcal{V}$ and weight parameters $\mathbf{w}$ are bounded by $B_x, B_w \geq 0$, i.e., $\| \mathbf{x}_i \|_2 \leq B_x,~\| \mathbf{w}\|_2 \leq B_w$.
\end{assumption}
% Moreover, we assume the variance of stochastic gradient is bounded.
\begin{assumption} \label{assumption:expectation_random_delete_nodes}
For any randomly selected deleted nodes set $\mathcal{V}_\text{delete}$, the variance of the stochastic gradient computed on the remaining nodes $\mathcal{V}_\text{remain} = \mathcal{V} \setminus \mathcal{V}_\text{delete}$ can be upper bounded by $G\geq0$, i.e., $\mathbb{E}_{\mathcal{V}_\text{delete}} \big[ \big\|  \frac{1}{|\mathcal{V}_\text{train}|}\sum\nolimits_{v_i\in\mathcal{V}_\text{train}} \nabla f_i^u(\mathbf{w}) - \frac{1}{|\mathcal{V}_\text{remain}|}\sum\nolimits_{v_i\in\mathcal{V}_\text{remain}} \nabla f_i^u(\mathbf{w}_u)  \big\|_2 \big] \leq G$.
% \begin{equation}
%     \mathbb{E}_{\mathcal{V}_\text{delete}} \left[ \left\|  \frac{1}{|\mathcal{V}_\text{train}|}\sum\nolimits_{i\in\mathcal{V}_\text{train}} \nabla f_i^u(\mathbf{w}) - \frac{1}{|\mathcal{V}_\text{remain}|}\sum\nolimits_{i\in\mathcal{V}_\text{remain}} \nabla f_i^u(\mathbf{w}_u) \mathbf{h}_i^u \right\|_2 \right] \leq G
% \end{equation}
\end{assumption}
\begin{assumption} \label{assumption:upper_bound_on_approximation_error}
For any node $v_j\in\mathcal{V}_\text{delete}$, its node feature $\mathbf{x}_j$ can be approximated by the linear combination of all node features in the remaining node set $\{\mathbf{x}_i~|~v_i\in\mathcal{V}_\text{remain}\}$ up to an error $\delta \geq 0$. Formally, we have $\max_{v_j\in\mathcal{V}_\text{delete}} \min_{\bm{\gamma}} \left\| \sum_{i\in\mathcal{V}_\text{remain}} \gamma_i \mathbf{x}_i - \mathbf{x}_j \right\|_2 \leq \delta$.
% \begin{equation}
%     \max_{j\in\mathcal{V}_\text{delete}} \min_{\bm{\gamma}} \left\| \sum_{i\in\mathcal{V}_\text{remain}} \gamma_i \mathbf{x}_i - \mathbf{x}_j \right\|_2 \leq \delta
% \end{equation}
\end{assumption}
Let us suppose the above assumptions hold, then we could show that the difference between $\mathbf{w}_p$ and $\mathbf{w}_u(T)$ is mainly controlled by three key factors: \circled{1} the difference between the propagation matrices before and after data deletion, which is captured by $P_d$ in Assumption~\ref{assumption:upper_bound_on_node_feats}; \circled{2} the closeness of any deleted node features that could be approximated by weighted combination of all node features in the remaining node sets, which is captured by $\delta$ in Assumption~\ref{assumption:upper_bound_on_approximation_error}; \circled{3} the variance of stochastic gradient computed on the remaining nodes, which is captured by $G$ in Assumption~\ref{assumption:expectation_random_delete_nodes}.
By reducing the number of nodes in $\mathcal{V}_\text{delete}$, all $P_d, \delta, G$ are expected to decrease.
At an extreme case where $\mathcal{V}_\text{delete}=\emptyset$, we have $P_d =\delta = G=0$ and  $\mathbf{w}_p=\mathbf{w}(T)=\mathbf{w}_u(T)$.
The proof is deferred to Appendix~\ref{section:proof_of_ell2_norm_of_weight_projections}.

\begin{theorem} \label{theorem:ell2_norm_of_weight_projections}
Let us suppose Assumptions~\ref{assumption:upper_bound_on_node_feats},\ref{assumption:upper_bound_on_approximation_error}, \ref{assumption:expectation_random_delete_nodes} hold and let us define $Q = \eta \big( (1+B_x B_w P_s) B_x P_d + G  \big)$ where $\eta$ is the learning rate used to pre-train the weight $\mathbf{w}(T)$ for $T$ steps of gradient descent updates. Then, 
% given \our weight parameters $\mathbf{w}(T)$ that has been trained by full-batch gradient descent for $T$ iterations, \our will output an unlearned weight parameter $\mathbf{w}_p(T)$, and 
the closeness of $\mathbf{w}_p$ to the weight parameters $\mathbf{w}_u(T)$ 
% obtained by retraining on the dataset after node deletion from scratch 
can be bounded by
\begin{equation}\label{eq:weight_diff_bound}
    \mathbb{E}_{\mathcal{V}_\text{delete}}[\| \mathbf{w}_u(T) - \mathbf{w}_p \|_2 ]
    \leq \Delta = Q \sum\nolimits_{t=1}^T \left(1+\eta (\lambda+B_x^2P_s^2)\right)^{t-1} + \delta \eta T \times |\mathcal{V}_\text{delete}|.
\end{equation}
% where $Q = \eta \big( (1+B_x B_w P_s) B_x P_d + G  \big)$.
After projection, we can finetune $\mathbf{w}_p$ for $K$ iterations with learning rate $(\lambda+B_x^{2} P_s^{2})^{-1}$ to obtain $\tilde{\mathbf{w}}_p$ that has an error
$F^u(\tilde{\mathbf{w}}_p) - \min_\mathbf{w} F^u(\mathbf{w}) \leq \mathcal{O}((\lambda+B^2_x P_s^2) \Delta / K)$
if $\mathbf{w}_u(T)$ closes to optimal.
% \begin{equation}
%     F_u(\mathbf{w}_p(K)) - \min_\mathbf{w} F_u(\mathbf{w}) \leq \mathcal{O}\left(\frac{(\lambda+B^2_x P_s^2) \Delta} { K-T}\right).
% \end{equation}
\end{theorem}

Besides, if $\delta$ satisfies the condition in Proposition~\ref{proposition:closeness_of_projector_vs_inflence}, we know the solution of \our is provably closer to the model retrained from scratch compared to~\cite{guo2020certified,golatkar2020eternal}. The condition is very likely to be satisfied because learning rate $\eta$, regularization term $\lambda$, and the ratio of deleted nodes $|\mathcal{V}_\text{delete}|/|\mathcal{V}|$ are usually small in practice.
Moreover, we empirically validate the difference between the weight before and after unlearning in the experiment section to validate our theoretical results. The proof of Proposition~\ref{proposition:closeness_of_projector_vs_inflence} is deferred to Appendix~\ref{section:proof_of_closeness_of_projector_vs_inflence}.

 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{proposition} \label{proposition:closeness_of_projector_vs_inflence}
If the approximation error in Assumption~\ref{assumption:upper_bound_on_approximation_error} satisfying $\delta  < \left((\lambda \eta T)^{-1} + 1 \right) B_x \times \frac{|\mathcal{V}|}{|\mathcal{V}_\text{delete}|}$, then the distance of \our is provably closer to re-training from scratch then using influence-based~\cite{guo2020certified} and Fisher-based~\cite{golatkar2020eternal} approximate unlearning methods.
\end{proposition}



==> sections/projector_logistic_regression.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Before introducing \our for graph representation unlearning, let us first consider logistic regression
$F(\mathbf{w})=\lambda\|\mathbf{w}\|_2^2/2 + \smash{ \sum_{i\in\mathcal{V}}} \log(1+\exp(-y_i \mathbf{w}^\top \mathbf{x}_i))$ 
to illustrate the key ideas. From the optimization theory, the optimal $\mathbf{w}$ is a linear combination of training instances with coefficient $\bm{\alpha} \in \mathbb{R}^{|\mathcal{V}|}$ and supporting vectors \smash{$\{\mathbf{x}_i\}_{v_i\in\mathcal{V}}$}, i.e., $\smash{\mathbf{w} = \sum_{v_i\in\mathcal{V}}  \alpha_i \mathbf{x}_i} \in \mathbb{R}^d$.
Let us suppose any node feature cannot be represented by linear combination of other node features and
% \footnote{Features independent refers to any feature cannot be represented by linear combination of other node features. This can be guaranteed by adding small random noise to features that does not hurt performance.} 
and we want to unlearn features $\mathbf{X}_\text{delete} = \{\mathbf{x}_i~|~v_i\in\mathcal{V}_\text{delete}\}$ of size $m=|\mathcal{V}_\text{delete}|$ by making sure $\mathbf{w}$ does not carry any information about $\mathbf{X}_\text{delete}$. 
Our main idea is to find an another linear combination by forcing  $\alpha_i=0$ for any $v_i\in\mathcal{V}_\text{delete}$.
This can be achieved by finding an alternative solution $\mathbf{w}_p$ from a subspace irrelevant to $\mathbf{X}_\text{delete}$ that is close to $\mathbf{w}$, i.e.,
$\mathbf{w}_p = \smash{{\arg\min}_{\mathbf{v}\in \text{span}\{ \mathbf{x}_i~|~v_i\in\mathcal{V}_\text{remain}\}}}~\| \mathbf{v} - \mathbf{w} \|_2^2$.
More specifically, let $\mathcal{U}$ denote the linear subspace  spanned by all remaining samples.
To obtain the optimal solution, we can orthogonal project $\mathbf{w}$ onto the subspace $\mathcal{U}$. Knowing that any projection $\Pi_\mathcal{U}(\mathbf{w})$ onto $\mathcal{U}$ is necessarily an element of $\mathcal{U}$, which can be represented as linear combination of $\{\mathbf{x}_i~|~v_i\in\mathcal{V}_\text{remain}\}$ such that $\smash{\Pi_\mathcal{U}(\mathbf{w}) = \sum_{v_i\in\mathcal{V}_\text{remain}} \alpha_i \mathbf{x}_i}$, where the coefficients of the orthogonal projection can be obtained by Proposition~\ref{proposition:projection_step}. An illustration of the projection-based unlearning is shown in Figure~\ref{fig:orthogonal_proj_weight} and the proof is provided in Appendix~\ref{section:proof_alternative_orthogonal_projection}.
% , the detailed algorithm in Algorithm~\ref{alg:projector}, .

\begin{proposition}\label{proposition:projection_step}
Let $\mathbf{X}_\text{remain} = \{\mathbf{x}_j~|~v_j\in\mathcal{V}_\text{remain}\}$ denote the stack of all remaining features of size $r=|\mathcal{V}_\text{remain}|$ after deletion and $\bm{\alpha} = \{\alpha_j~|~ v_j\in\mathcal{V}_\text{remain}\}$ as the vectorized coefficients, which could be computed by $\bm{\alpha} = \mathbf{X}_\text{remain} (\mathbf{X}_\text{remain}^\top \mathbf{X}_\text{remain} )^\dagger \mathbf{w}$, where $\dagger$ denotes pseudo-inverse. 
\end{proposition}

% The above result shows that we can find the coefficients of the orthogonal projection by using the right pseudo-inverse of the remaining features.
The significant  computation required in Proposition~\ref{proposition:projection_step} includes 
computing $\mathbf{X}_\text{remain}^\top \mathbf{X}_\text{remain}\in \mathbb{R}^{d \times d}$ and its inverse with $\mathcal{O}(r d^2)$ and $\mathcal{O}(d^3)$ computation complexity, respectively.
However, if we suppose $\mathbf{X}^\top \mathbf{X}$ can be pre-computed before the unlearning request is made,
under the circumstance that not all remaining node features are available during unlearning, one can still compute $\mathbf{X}_\text{remain}^\top \mathbf{X}_\text{remain}$ by  $\mathbf{X}^\top \mathbf{X} - \mathbf{X}_\text{delete}^\top \mathbf{X}_\text{delete}$ and compute $(\mathbf{X}_\text{remain}^\top \mathbf{X}_\text{remain})^\dagger$ by applying the Woodbury identity~\cite{golub2013matrix} on $\mathbf{X}_\text{delete}^\top \mathbf{X}_\text{delete}$ and $\mathbf{X}^\top \mathbf{X}$, which leads to a lower computation complexity of $\mathcal{O}(\max\{m^3, m d^2\})$ if $m < \max\{r,d\}$.
After obtaining $\bm{\alpha}$, \our computes the unlearned weight parameters by $\mathbf{w}_p = \mathbf{X}_\text{remain}^\top \bm{\alpha}$.
% Let $\mathbf{w}_u$ denote the optimal weight on the dataset after data deletion.
% Under the assumption that small perturbation on the dataset will not affect the optimal weight much, as shown in Figure~\ref{fig:unleaning_ERM}, we expect $\mathbf{w}_p, \mathbf{w} $ are closed to $\mathbf{w}_u$. 
% Therefore, one can take $\mathbf{w}_p$ as an initialization and finetune for several iterations to boost the performance.
Besides, 
due to the similarity between logistic regression to SVM, 
\our is also applicable to primal-based SVM unlearning to alleviate the high computation cost
% of iterative optimality condition maintaining steps 
in the dual-based SVM unlearning approach~\cite{cauwenberghs2000incremental}.
Readers who are also interested in its application on SVM could refer to Appendix~\ref{section:connection_to_svm} for details.
In the next section, we will introduce the application of \our onto graph representation unlearning and explain why \our could bypass the node dependency issue in graph structured data.



==> tables/delete_data_reply_test_cora.tex <==
\begin{table}[t]
\centering
\caption{Comparison on the \textit{F1-score accuracy} (\textcolor{brown}{Accuracy}),
% the number of the delete nodes that are predicted as the extra-label category (\textcolor{cyan}{Num delete}),
and the norm of extra-feature weight channel (\textcolor{cyan}{Weight norm}) before unlearning and after unlearning (denoted as \textit{before} $\rightarrow$ \textit{after}), and wall-clock time (\textcolor{teal}{Time}) using linear GNN. ``-'' stands for cannot generate meaningful results.}
\label{table:feature_injection_test_cora}
\vspace{-3mm}
\resizebox{\textwidth}{2cm}{
\begin{tabular}{l l l l l l}
\hline\hline \rule{0pt}{2ex}   
                                       & Method                & Metrics  & Delete $2\%$ nodes           & Delete $5\%$ nodes           & Delete $10\%$ nodes        \\ \hline\hline \rule{0pt}{2ex}   
% \multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{OGB-Arxiv}}}    
%                                       & \cellcolor[HTML]{FEDEDC} & \cellcolor[HTML]{FEDEDC}\textcolor{brown}{Accuracy} (\%)      & \cellcolor[HTML]{FEDEDC}$73.39\rightarrow 73.32$       & \cellcolor[HTML]{FEDEDC}$73.33\rightarrow 73.39$       & \cellcolor[HTML]{FEDEDC}$73.25\rightarrow 73.39$     \\ 
%                                       & \cellcolor[HTML]{FEDEDC}\multirow{-2}{*}{\our}  & \cellcolor[HTML]{FEDEDC}\textcolor{cyan}{Weight norm} (\textcolor{teal}{Time}) & \cellcolor[HTML]{FEDEDC}$19.4\rightarrow 0$~($0.07$ s)   & \cellcolor[HTML]{FEDEDC}$21.7 \rightarrow 0$~($0.07$ s)   & \cellcolor[HTML]{FEDEDC}$56.8 \rightarrow 0$~($0.07$ s) \\
%                                       \cline{2-6} \rule{0pt}{2ex}   
%                                       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       & \cellcolor[HTML]{C4F8F6} & \cellcolor[HTML]{C4F8F6}\textcolor{brown}{Accuracy} (\%)         & \cellcolor[HTML]{C4F8F6}$73.44\rightarrow 73.52$         & \cellcolor[HTML]{C4F8F6}$73.42\rightarrow 73.48$         & \cellcolor[HTML]{C4F8F6}$73.34\rightarrow 73.44$     \\ 
%                                       & \cellcolor[HTML]{C4F8F6}\multirow{-2}{*}{\cellcolor[HTML]{C4F8F6}\begin{tabular}[c]{@{}l@{}} \our \\ (+ adapt diff) \end{tabular}}  & \cellcolor[HTML]{C4F8F6}\textcolor{cyan}{Weight norm} (\textcolor{teal}{Time}) & \cellcolor[HTML]{C4F8F6}$21.0\rightarrow 0$~($0.07$ s)   & \cellcolor[HTML]{C4F8F6}$24.3 \rightarrow 0$~($0.07$ s)   & \cellcolor[HTML]{C4F8F6}$25.6 \rightarrow 0$~($0.07$ s) \\ \cline{2-6} \rule{0pt}{2ex}  
%                                       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}} \textsc{GraphEraser} \\ ($\times 8$ subgraphs) \end{tabular}} 
%                                                               & \textcolor{brown}{Accuracy} (\%)      & $70.67\rightarrow 70.66$       & $70.59\rightarrow 70.56$       & $70.55\rightarrow 70.23$      \\ 
%                                       &                       & \textcolor{cyan}{Weight norm} (\textcolor{teal}{Time}) & $21.4 \rightarrow 0$~($1,866\times8$ s)   & $22.3 \rightarrow 0$~($1,866\times8$ s)   & $30.6 \rightarrow 0$~($1,866\times8$ s) \\\cline{2-6} \rule{0pt}{2ex}    
%                                       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       & \multirow{2}{*}{\textsc{Influence}+} 
%                                                               & \textcolor{brown}{Accuracy} (\%)      & $71.68\rightarrow 72.49$       & $71.90\rightarrow 72.73$       & $ 70.40 \rightarrow 72.65 $     \\ 
%                                       &                       & \textcolor{cyan}{Weight norm} (\textcolor{teal}{Time}) & $21.1 \rightarrow 12.4$~($1.1$ s)   & $29.2 \rightarrow 14.1$~($1.1$ s)   & $21.1 \rightarrow 12.1$~($1.1$ s) \\\cline{2-6} \rule{0pt}{2ex}    
%                                     %   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                     %   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                     %   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       & \multirow{2}{*}{\textsc{Fisher}+} 
%                                                               & \textcolor{brown}{Accuracy} (\%)      & $72.44\rightarrow 72.49$       & $72.29\rightarrow 72.73$       & $ 71.71 \rightarrow 72.65 $     \\ 
%                                       &                       & \textcolor{cyan}{Weight norm} (\textcolor{teal}{Time}) & $21.1 \rightarrow 12.4$~($0.6$ s)   & $29.2 \rightarrow 14.1$~($0.4$ s)   & $35.4 \rightarrow 15.6$~($0.3$ s) \\ \hline\hline \rule{0pt}{2ex}    
% \multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{OGB-Products}}}    
%                                       & \cellcolor[HTML]{FEDEDC} & \cellcolor[HTML]{FEDEDC}\textcolor{brown}{Accuracy} (\%)      & \cellcolor[HTML]{FEDEDC}$79.08\rightarrow 79.10$       & \cellcolor[HTML]{FEDEDC}$79.21\rightarrow 79.22$       & \cellcolor[HTML]{FEDEDC}$79.18\rightarrow 79.11$     \\ 
%                                       & \cellcolor[HTML]{FEDEDC}\multirow{-2}{*}{\our}  & \cellcolor[HTML]{FEDEDC}\textcolor{cyan}{Weight norm} (\textcolor{teal}{Time}) & \cellcolor[HTML]{FEDEDC}$21.1\rightarrow 0$~($0.06$ s)   & \cellcolor[HTML]{FEDEDC}$27.6 \rightarrow 0$~($0.06$ s)   & \cellcolor[HTML]{FEDEDC}$30.8 \rightarrow 0$~($0.06$ s) \\
%                                       \cline{2-6} \rule{0pt}{2ex}   
%                                       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       & \cellcolor[HTML]{C4F8F6} & \cellcolor[HTML]{C4F8F6}\textcolor{brown}{Accuracy} (\%)         & \cellcolor[HTML]{C4F8F6}$79.81\rightarrow 79.79$         & \cellcolor[HTML]{C4F8F6}$79.95\rightarrow 79.93$         & \cellcolor[HTML]{C4F8F6}$79.96\rightarrow 79.91$     \\ 
%                                       & \cellcolor[HTML]{C4F8F6}\multirow{-2}{*}{\cellcolor[HTML]{C4F8F6}\begin{tabular}[c]{@{}l@{}} \our \\ (+ adapt diff) \end{tabular}}  & \cellcolor[HTML]{C4F8F6}\textcolor{cyan}{Weight norm} (\textcolor{teal}{Time}) & \cellcolor[HTML]{C4F8F6}$13.3\rightarrow 0$~($0.06$ s)   & \cellcolor[HTML]{C4F8F6}$16.4 \rightarrow 0$~($0.06$ s)   & \cellcolor[HTML]{C4F8F6}$18.6\rightarrow 0$~($0.06$ s) \\ \cline{2-6} \rule{0pt}{2ex}  
%                                       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}} \textsc{GraphEraser} \\ ($\times 8$ subgraphs) \end{tabular}} 
%                                                               & \textcolor{brown}{Accuracy} (\%)      & $70.79\rightarrow 70.78$       & $70.80\rightarrow 70.78$       & $70.80\rightarrow 70.78$     \\ 
%                                       &                       & \textcolor{cyan}{Weight norm} (\textcolor{teal}{Time}) & $21.4 \rightarrow 0$~($598\times8$ s)   & $25.4 \rightarrow 0$~($598\times8$ s)   & $28.9 \rightarrow 0$~($598\times8$ s) \\\cline{2-6} \rule{0pt}{2ex}    
%                                       & \multirow{2}{*}{\textsc{Influence}+} 
%                                                               & \textcolor{brown}{Accuracy} (\%)      & $72.28\rightarrow 72.58$       & $72.23\rightarrow 72.78$       & $ 72.08 \rightarrow 72.51 $     \\ 
%                                       &                       & \textcolor{cyan}{Weight norm} (\textcolor{teal}{Time}) & $4.4 \rightarrow 1.8$~($1.6$ s)   & $8.9 \rightarrow 3.1$~($1.7$ s)   & $14.3 \rightarrow 4.2$~($1.9$ s) \\\cline{2-6} \rule{0pt}{2ex}    
%                                       & \multirow{2}{*}{\textsc{Fisher}+} 
%                                                               & \textcolor{brown}{Accuracy} (\%)      & $72.28\rightarrow 72.54$       & $72.23\rightarrow 72.78$       & $ 72.08 \rightarrow 72.51 $     \\ 
%                                       &                       & \textcolor{cyan}{Weight norm} (\textcolor{teal}{Time}) & $4.4 \rightarrow 1.8$~($1.6$ s)   & $8.9 \rightarrow 3.1$~($1.3$ s)   & $14.3 \rightarrow 4.2$~($1.1$ s) \\ \cline{2-6} 
%                                       \hline\hline \rule{0pt}{2ex}   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Cora}}}    
                                      & \cellcolor[HTML]{FEDEDC} & \cellcolor[HTML]{FEDEDC}\textcolor{brown}{Accuracy} (\%)      & \cellcolor[HTML]{FEDEDC}$77.2\rightarrow 77.1$       & \cellcolor[HTML]{FEDEDC}$77.3\rightarrow 76.8$       & \cellcolor[HTML]{FEDEDC}$75.5\rightarrow 76.1$     \\ 
                                      & \cellcolor[HTML]{FEDEDC}\multirow{-2}{*}{\our}  & \cellcolor[HTML]{FEDEDC}\textcolor{cyan}{Weight norm} (\textcolor{teal}{Time}) & \cellcolor[HTML]{FEDEDC}$2.3\rightarrow 0$~($0.13$ s)   & \cellcolor[HTML]{FEDEDC}$4.1 \rightarrow 0$~($0.13$ s)   & \cellcolor[HTML]{FEDEDC}$5.5 \rightarrow 0$~($0.13$ s) \\
                                      \cline{2-6} \rule{0pt}{2ex}   
                                      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                                      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                                      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                                      & \multirow{2}{*}{\textsc{Influence}+} 
                                                              & \textcolor{brown}{Accuracy} (\%)      & $73.1\rightarrow 59.0$       & $ - $       & $ - $     \\ 
                                      &                       & \textcolor{cyan}{Weight norm} (\textcolor{teal}{Time}) & $0.81 \rightarrow 0.59$~($0.2$ s)   & $-$  & $ - $ \\\cline{2-6} \rule{0pt}{2ex}    
                                    %   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                                    %   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                                    %   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                                      & \multirow{2}{*}{\textsc{Fisher}+} 
                                                              & \textcolor{brown}{Accuracy} (\%)      & $73.1\rightarrow 73.6$       & $72.0\rightarrow 72.7$       & $ 72.0 \rightarrow 72.4 $     \\ 
                                      &                       & \textcolor{cyan}{Weight norm} (\textcolor{teal}{Time}) & $0.81 \rightarrow 0.08$~($0.19$ s)   & $0.72 \rightarrow 0.08$~($0.19$ s)   & $0.78\rightarrow 0.18$~($0.19$ s) \\ \hline\hline \rule{0pt}{2ex} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Citeseer}}}    
%                                       & \cellcolor[HTML]{FEDEDC} & \cellcolor[HTML]{FEDEDC}\textcolor{brown}{Accuracy} (\%)      & \cellcolor[HTML]{FEDEDC}$75.7\rightarrow 75.7$       & \cellcolor[HTML]{FEDEDC}$75.3\rightarrow 75.5$       & \cellcolor[HTML]{FEDEDC}$74.4\rightarrow 74.1$     \\ 
%                                       & \cellcolor[HTML]{FEDEDC}\multirow{-2}{*}{\our}  & \cellcolor[HTML]{FEDEDC}\textcolor{cyan}{Weight norm} (\textcolor{teal}{Time}) & \cellcolor[HTML]{FEDEDC}$1.15\rightarrow 0$~($4.1$ s)   & \cellcolor[HTML]{FEDEDC}$2.6 \rightarrow 0$~($4.1$ s)   & \cellcolor[HTML]{FEDEDC}$3.4 \rightarrow 0$~($4.1$ s) \\  \cline{2-6} \rule{0pt}{2ex}   
%                                       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       & \multirow{2}{*}{\textsc{Influence}+} & \textcolor{brown}{Accuracy} (\%)      & $73.7 \rightarrow 70.0$       & $ - $       & $ - $     \\ 
%                                       &                                      & \textcolor{cyan}{Weight norm} (\textcolor{teal}{Time}) & $0.23 \rightarrow 0.47$~($1.5$ s)   & $-$  & $ - $ \\\cline{2-6} \rule{0pt}{2ex}    
%                                     %   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                     %   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                     %   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       & \multirow{2}{*}{\textsc{Fisher}+} & \textcolor{brown}{Accuracy} (\%)      & $73.7\rightarrow 75.4$       & $73.8\rightarrow 75.6$       & $ 73.7 \rightarrow 75.9 $     \\ 
%                                       &                                   & \textcolor{cyan}{Weight norm} (\textcolor{teal}{Time}) & $0.23 \rightarrow 0.05$~($1.4$ s)   & $0.24 \rightarrow 0.1$~($1.4$ s)   & $0.18 \rightarrow 0.18$~($1.4$ s)\\ \hline\hline \rule{0pt}{2ex} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Pubmed}}}    
                                      & \cellcolor[HTML]{FEDEDC} & \cellcolor[HTML]{FEDEDC}\textcolor{brown}{Accuracy} (\%)      & \cellcolor[HTML]{FEDEDC}$86.1\rightarrow 86.1$       & \cellcolor[HTML]{FEDEDC}$86.3\rightarrow 86.3$       & \cellcolor[HTML]{FEDEDC}$86.7\rightarrow 86.7$     \\ 
                                      & \cellcolor[HTML]{FEDEDC}\multirow{-2}{*}{\our}  & \cellcolor[HTML]{FEDEDC}\textcolor{cyan}{Weight norm} (\textcolor{teal}{Time}) & \cellcolor[HTML]{FEDEDC}$9.1\rightarrow 0$~($0.03$ s)   & \cellcolor[HTML]{FEDEDC}$10.1 \rightarrow 0$~($0.03$ s)   & \cellcolor[HTML]{FEDEDC}$11.1 \rightarrow 0$~($0.03$ s) \\  \cline{2-6} \rule{0pt}{2ex}   
                                      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                                      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                                      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                                      & \multirow{2}{*}{\textsc{Influence}+} & \textcolor{brown}{Accuracy} (\%)      & $80.8 \rightarrow 82.4$       & $80.9 \rightarrow 82.8$       & $80.6 \rightarrow 82.2$     \\ 
                                      &                                      & \textcolor{cyan}{Weight norm} (\textcolor{teal}{Time}) & $4.6 \rightarrow 4.7$~($1.18$ s)   & $5.9 \rightarrow 10.0$~($1.18$ s)  & $7.0 \rightarrow 29.1$~($1.18$ s) \\\cline{2-6} \rule{0pt}{2ex}    
                                    %   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                                    %   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                                    %   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                                      & \multirow{2}{*}{\textsc{Fisher}+} & \textcolor{brown}{Accuracy} (\%)      & $83.3 \rightarrow 83.2$       & $83.7 \rightarrow 84.8$       & $83.7 \rightarrow 84.7$     \\ 
                                      &                                      & \textcolor{cyan}{Weight norm} (\textcolor{teal}{Time}) & $9.1 \rightarrow 0.6$~($1.17$ s)   & $10.7 \rightarrow 1.6$~($1.16$ s)  & $10.9 \rightarrow 2.6$~($1.15$ s) \\ \hline\hline \rule{0pt}{2ex} 
\end{tabular}
}
% \vspace{-5mm}
\end{table}


% influence based training time: 
% retraining linear GNN 1,335 sec


